Convex Hull Approximation of Nearly Optimal Lasso Solutions

In an ordinary feature selection procedure, a set of important features is obtained by solving an optimization problem such as the Lasso regression problem, and we expect that the obtained features explain the data well. In this study, instead of the single optimal solution, we consider finding a set of diverse yet nearly optimal solutions. To this end, we formulate the problem as finding a small number of solutions such that the convex hull of these solutions approximates the set of nearly optimal solutions. The proposed algorithm consists of two steps: First, we randomly sample the extreme points of the set of nearly optimal solutions. Then, we select a small number of points using a greedy algorithm. The experimental results indicate that the proposed algorithm can approximate the solution set well. The results also indicate that we can obtain Lasso solutions with a large diversity.

==> additional_experiments.tex <==
\section{Additional Results}
\label{app:add_results}

We have evaluated the efficacy of the proposed method on some of libsvm datasets\footnote{\url{https://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/}}: we used \texttt{cputime} for regression \eqref{eq:L}, and \texttt{australian}, \texttt{german.numer}, \texttt{ionosphere}, \texttt{sonar}, and \texttt{splice} for binary classification \eqref{eq:logreg}.
In the experiments, we searched for 50 near optimal solutions using the proposed method where we set $\nu = 1.05 L(\beta^*)$ and the number of samplings $M=1,000$.
We also enumerated 50 solutions using the two baselines, Enumeration and Heuristics (see Section~\ref{sec:diversity}).

The results are shown in \figurename~\ref{fig:add_results}.
For regression, we set $\rho = 0.1$, and for binary classification, we set $\rho = 0.01$, so that the solutions to be sufficiently sparse.
In the figures, similar to the results in Section~\ref{sec:diversity}, we have projected the solutions into two dimensional space using PCA.
The figures show the clear advantage of the proposed method in that it can find solutions with large diversities compared to the exhaustive enumerations.

\begin{figure*}[!ht]
	\centering
	\begin{minipage}[t]{0.3\textwidth}
	\begin{tikzpicture}
		\node[above right] (img) at (0,0) {\includegraphics[width=0.96\textwidth]{cpusmall_diversity.pdf}};
		\draw [very thin] (0.97, 4.69) rectangle (3.16, 5.74);
		\node[circle, draw=red, fill=white, inner sep=0pt, minimum size=5pt, line width=1pt] (a) at (34pt, 158pt) {};
		\node[rectangle, draw={rgb:green,5;blue,2;red,2}, fill={rgb:green,2;white,1}, inner sep=0pt, minimum size=5pt, line width=1pt] (b) at (34pt, 148pt) {};
		\node[text=blue] (c) at (34pt, 138pt) {+};
		\node[right] at (38pt, 158pt) {\footnotesize Enumeration};
		\node[right] at (38pt, 148pt) {\footnotesize Heuristic};
		\node[right] at (38pt, 138pt) {\footnotesize Proposed};
	\end{tikzpicture}
	\subcaption{cputime}
	\label{fig:cpusmall_diversity}
	\end{minipage}
    	\hfill
	\begin{minipage}[t]{0.3\textwidth}
	\begin{tikzpicture}
		\node[above right] (img) at (0,0) {\includegraphics[width=0.96\textwidth]{australian_diversity.pdf}};
		%\draw [very thin] (1.97, 0.69) rectangle (4.16, 1.74);
		%\node[circle, draw=red, fill=white, inner sep=0pt, minimum size=5pt, line width=1pt] (a) at (62pt, 45pt) {};
		%\node[rectangle, draw={rgb:green,5;blue,2;red,2}, fill={rgb:green,2;white,1}, inner sep=0pt, minimum size=5pt, line width=1pt] (b) at (62pt, 35pt) {};
		%\node[text=blue] (c) at (62pt, 25pt) {+};
		%\node[right] at (66pt, 45pt) {\footnotesize Enumeration};
		%\node[right] at (66pt, 35pt) {\footnotesize Heuristic};
		%\node[right] at (66pt, 25pt) {\footnotesize Proposed};
	\end{tikzpicture}
	\subcaption{australian}
	\label{fig:australian_diversity}
	\end{minipage}
    	\hfill
    	\begin{minipage}[t]{0.3\textwidth}
	\begin{tikzpicture}
		\node[above right] (img) at (0,0) {\includegraphics[width=0.96\textwidth]{german_numer_diversity.pdf}};
		%\draw [very thin] (1.97, 0.69) rectangle (4.16, 1.74);
		%\node[circle, draw=red, fill=white, inner sep=0pt, minimum size=5pt, line width=1pt] (a) at (62pt, 45pt) {};
		%\node[rectangle, draw={rgb:green,5;blue,2;red,2}, fill={rgb:green,2;white,1}, inner sep=0pt, minimum size=5pt, line width=1pt] (b) at (62pt, 35pt) {};
		%\node[text=blue] (c) at (62pt, 25pt) {+};
		%\node[right] at (66pt, 45pt) {\footnotesize Enumeration};
		%\node[right] at (66pt, 35pt) {\footnotesize Heuristic};
		%\node[right] at (66pt, 25pt) {\footnotesize Proposed};
	\end{tikzpicture}
	\subcaption{german.numer}
	\label{fig:german_numer_diversity}
	\end{minipage}\\
    	\begin{minipage}[t]{0.3\textwidth}
	\begin{tikzpicture}
		\node[above right] (img) at (0,0) {\includegraphics[width=0.96\textwidth]{ionosphere_diversity.pdf}};
		%\draw [very thin] (1.97, 0.69) rectangle (4.16, 1.74);
		%\node[circle, draw=red, fill=white, inner sep=0pt, minimum size=5pt, line width=1pt] (a) at (62pt, 45pt) {};
		%\node[rectangle, draw={rgb:green,5;blue,2;red,2}, fill={rgb:green,2;white,1}, inner sep=0pt, minimum size=5pt, line width=1pt] (b) at (62pt, 35pt) {};
		%\node[text=blue] (c) at (62pt, 25pt) {+};
		%\node[right] at (66pt, 45pt) {\footnotesize Enumeration};
		%\node[right] at (66pt, 35pt) {\footnotesize Heuristic};
		%\node[right] at (66pt, 25pt) {\footnotesize Proposed};
	\end{tikzpicture}
	\subcaption{ionosphere}
	\label{fig:ionosphere_diversity}
	\end{minipage}
    	\hfill
    	\begin{minipage}[t]{0.3\textwidth}
	\begin{tikzpicture}
		\node[above right] (img) at (0,0) {\includegraphics[width=0.96\textwidth]{sonar_diversity.pdf}};
		%\draw [very thin] (1.97, 0.69) rectangle (4.16, 1.74);
		%\node[circle, draw=red, fill=white, inner sep=0pt, minimum size=5pt, line width=1pt] (a) at (62pt, 45pt) {};
		%\node[rectangle, draw={rgb:green,5;blue,2;red,2}, fill={rgb:green,2;white,1}, inner sep=0pt, minimum size=5pt, line width=1pt] (b) at (62pt, 35pt) {};
		%\node[text=blue] (c) at (62pt, 25pt) {+};
		%\node[right] at (66pt, 45pt) {\footnotesize Enumeration};
		%\node[right] at (66pt, 35pt) {\footnotesize Heuristic};
		%\node[right] at (66pt, 25pt) {\footnotesize Proposed};
	\end{tikzpicture}
	\subcaption{sonar}
	\label{fig:sonar_diversity}
	\end{minipage}
    	\hfill
    	\begin{minipage}[t]{0.3\textwidth}
	\begin{tikzpicture}
		\node[above right] (img) at (0,0) {\includegraphics[width=0.96\textwidth]{splice_diversity.pdf}};
		%\draw [very thin] (1.97, 0.69) rectangle (4.16, 1.74);
		%\node[circle, draw=red, fill=white, inner sep=0pt, minimum size=5pt, line width=1pt] (a) at (62pt, 45pt) {};
		%\node[rectangle, draw={rgb:green,5;blue,2;red,2}, fill={rgb:green,2;white,1}, inner sep=0pt, minimum size=5pt, line width=1pt] (b) at (62pt, 35pt) {};
		%\node[text=blue] (c) at (62pt, 25pt) {+};
		%\node[right] at (66pt, 45pt) {\footnotesize Enumeration};
		%\node[right] at (66pt, 35pt) {\footnotesize Heuristic};
		%\node[right] at (66pt, 25pt) {\footnotesize Proposed};
	\end{tikzpicture}
	\subcaption{splice}
	\label{fig:splice_diversity}
	\end{minipage}
	\caption{Found 50 solutions, shown in 2D using PCA}
	\label{fig:add_results}
\end{figure*}
